GraphiQ: Quantum circuit design for photonic graph states

GraphiQ is a versatile open-source framework for designing photonic graph state generation schemes, with a particular emphasis on photon-emitter hybrid circuits. Built in Python, GraphiQ consists of a suite of design tools, including multiple simulation backends and optimization methods. The library supports scheme optimization in the presence of circuit imperfections, as well as user-defined optimization goals. Our framework thus represents a valuable tool for the development of practical schemes adhering to experimentally-relevant constraints. As graph states are a key resource for measurement-based quantum computing, all-photonic quantum repeaters, and robust quantum metrology, among others, we envision GraphiQ's broad impact for advancing quantum technologies.

==> code/metrics.tex <==
from graphiq.metrics import Fidelity, EmitterDepth

graph = nx.grid_graph((2, 2))
target = QuantumState(n=4, data=graph)

backend = DMBackend()
state = backend.run(circuit)

fidelity = Fidelity().evaluate(state, target)
depth = EmitterDepth().evaluate(circuit)



